PatchEX: High-Quality Real-Time Temporal Supersampling through Patch-based Parallel Extrapolation

High-refresh rate displays have become very popular in recent years due to the need for superior visual quality in gaming, professional displays and specialized applications like medical imaging. However, high-refresh rate displays alone do not guarantee a superior visual experience; the GPU needs to render frames at a matching rate. Otherwise, we observe disconcerting visual artifacts such as screen tearing and stuttering. Temporal supersampling is an effective technique to increase frame rates by predicting new frames from other rendered frames. There are two methods in this space: interpolation and extrapolation. Interpolation-based methods provide good image quality at the cost of a higher latency because they also require the next rendered frame. On the other hand, extrapolation methods are much faster at the cost of quality. This paper introduces PatchEX, a novel frame extrapolation method that aims to provide the quality of interpolation at the speed of extrapolation. It smartly partitions the extrapolation task into sub-tasks and executes them in parallel to improve both quality and latency. It then uses a patch-based inpainting method and a custom shadow prediction approach to fuse the generated sub-frames. This approach significantly reduces the overall latency while maintaining the quality of the output. Our results demonstrate that PatchEX achieves a 65.29% and 48.46% improvement in PSNR over the latest extrapolation methods ExtraNet and ExtraSS, respectively, while being 6x and 2x faster, respectively.

==> background.tex <==
\section{Background}
\label{sec:Background}

\subsection{Interpolation Vs Extrapolation}
\label{subsubsec:inter_vs_extra}

\textit{Interpolation} predicts frames between two already rendered neighboring frames, while \textit{extrapolation}
predicts frames solely based on past frames. In Figure~\ref{inter_vs_extra}, we observe that both interpolation and
extrapolation introduce some latency in the system, which is their own operational latency. Both processes double the
frame rate by generating a new frame after each rendered frame and display the frame in the following order $0, 0.5, 1,
1.5, 2, ..$. However, interpolation introduces an additional latency because it buffers an already rendered frame $F$, starts
the interpolation, displays the interpolated frame, and then displays frame $F$.

% Let us consider the newly generated frame with suffix $1.5$. In interpolation, the frame $I_{1.5}$  is generated using two frames $F_1$ and $F_2$. Since frame $I_{1.5}$ needs to be displayed before $F_2$, it waits for $F_2$, holds it, starts interpolating $I_{0.5}$, and first displays the interpolated frame, and then $F_2$. Hence, the input latency becomes interpolation cost + the time before displaying $F_2$. Whereas in the case of extrapolation, the new frame, $E_{1.5}$ is generated only based on the past frame $F_1$ and all the frames are displayed at the very next refresh cycle.

\begin{figure*}[!htbp]
	\centering
	\includegraphics[width=0.55\textwidth]{FIGS/int_vs_exr.pdf}
	\caption{Interpolation and extrapolation explained. 
$F_1$, $F_2$, $F_3$ and $F_4$ are frames. $I$ and $E$ stand for interpolation and extrapolation, respectively.}
	\label{inter_vs_extra}
\end{figure*}

\subsection{Reinforcement Learning (RL)}
\label{RL}
Reinforcement Learning (RL)~\cite{sutton1999reinforcement} is a machine learning-based technique that allows an agent to
learn how to make decisions in an uncertain environment by using feedback from its actions. It doesn't need labeled data.
The problem needs to be defined with a state space (set of all states based on observable variables), action space and rewards
(each rewards corresponds to a $\langle state,action\, pair \rangle$ that is not known a priori).  Now, given that the full state of the system 
is not fully visible to the agent, the state itself embeds a degree of uncertainty. As a result, any action on the state
also has an uncertain outcome in terms of the next state and the reward. The uncertainty is an inherent property of the 
environment. Gradually, over many cycles the agent learns more and more about the reward and state transition functions
using a learning-based approach. Once this process of training is over, the agent can make a good guess regarding the best
action for a given state, where the explicit aim is to maximize the reward. 

